The landscapemetrics and motif packages for measuring landscape patterns and processes

This book chapter emphasizes the significance of categorical raster data in ecological studies, specifically land use or land cover (LULC) data, and highlights the pivotal role of landscape metrics and pattern-based spatial analysis in comprehending environmental patterns and their dynamics. It explores the usage of R packages, particularly landscapemetrics and motif, for quantifying and analyzing landscape patterns using LULC data from three distinct European regions. It showcases the computation, visualization, and comparison of landscape metrics, while also addressing additional features such as patch value extraction, sub-region sampling, and moving window computation. Furthermore, the chapter delves into the intricacies of pattern-based spatial analysis, explaining how spatial signatures are computed and how the motif package facilitates comparisons and clustering of landscape patterns. The chapter concludes by discussing the potential of customization and expansion of the presented tools.

==> title.tex <==
$if(title)$
\title{$title$$if(thanks)$\thanks{$thanks$}$endif$}
$endif$

$if(subtitle)$
\subtitle{$subtitle$}
$endif$

$for(by-author)$
  \author{$by-author.name.literal$}
  $if(by-author.affiliations)$
    $for(by-author.affiliations)$
      \affil{%
        $if(by-author.affiliations.name)$
          $by-author.affiliations.name$
        $endif$
      }
    $endfor$
  $endif$
$endfor$

\date{$date$}
